Sparse SPN: Depth Completion from Sparse Keypoints

Our long term goal is to use image-based depth completion to quickly create 3D models from sparse point clouds, e.g. from SfM or SLAM. Much progress has been made in depth completion. However, most current works assume well distributed samples of known depth, e.g. Lidar or random uniform sampling, and perform poorly on uneven samples, such as from keypoints, due to the large unsampled regions. To address this problem, we extend CSPN with multiscale prediction and a dilated kernel, leading to much better completion of keypoint-sampled depth. We also show that a model trained on NYUv2 creates surprisingly good point clouds on ETH3D by completing sparse SfM points.

==> tables/eth3d_depth.tex <==
\begin{table}
\vspace{-0.05in}
\centering
    \resizebox{!}{10mm}{
    \begin{tabular}{c|cc|cccc}
    \toprule
    Method  & RMSE & REL & $\delta_{1.02}$ & $\delta_{1.05}$ & $\delta_{1.10}$ & $\delta_{1.25}$  \\ 
    \midrule
    CSPN ~\cite{cspn}     & 2.20           & 0.160          & 32.6          & 50.1          & 62.6          & 77.6          \\
    NLSPN ~\cite{nlspn}   & \textbf{1.82}  & 0.158          & 43.3          & 59.2          & 71.0          & 84.1          \\ 
    Ours - w/o normals                  & 5.18           & \textbf{0.130} & 47.5 & \textbf{62.9} & \textbf{73.6} & \textbf{85.5} \\ 
    Ours                  & 3.51           & 0.159 & \textbf{47.9} & 62.5 & 72.4 & 83.9 \\     

    
    \bottomrule
\end{tabular}
}
\caption{\small{\textbf{ETH3D High-Res Multi-View Training set Depth evaluation Results.} 
    Numbers in bold refers to the best results per different settings. }
}
\label{tab:eth3d_depth}
\end{table}

==> tables/eth3d_depth_replaced.tex <==
\begin{table}
\centering
\resizebox{83.5mm}{!}{
    \begin{tabular}{c|cc|cccc}
    \toprule
    Method  & RMSE & REL & $\delta_{1.02}$ & $\delta_{1.05}$ & $\delta_{1.10}$ & $\delta_{1.25}$  \\ 
    \midrule
    CSPN ~\cite{cspn}     & 2.19           & 0.146          & 33.9          & 50.7          & 62.8          & 77.5          \\
    NLSPN ~\cite{nlspn}   & 1.20  & 0.093          & 46.9          & 63.0          & 74.6          & \textbf{87.2}          \\ 
    Ours                  & \textbf{1.10}           & \textbf{0.089} & \textbf{50.7} & \textbf{65.7} & \textbf{76.1} & 87.0 \\ 
    \bottomrule
\end{tabular}
}
\caption{\textbf{ETH3D Depth Evaluation} with correct input values. 
We 
Numbers in bold refers to the best results per different settings. 
}
\label{tab:eth3d_depth_replaced}
\end{table}

==> tables/kitti_whole_table/kitti_keypoint.tex <==

\multirow{3}{*}{Keypoint} & CSPN   & ? & ? & ? & ? \\
 & NLSPN   & ? & ? & ? & ? \\
 & Ours & ? & ? & ? & ? \\\hline


==> tables/kitti_whole_table/kitti_lidar.tex <==

\multirow{3}{*}{Lidar} & CSPN  & ? & ? & ? & ?  \\
& NLSPN  & ? & ? & ? & ?  \\ 
 & Ours & ? & ? & ? & ? \\ \hline


==> tables/kitti_whole_table/kitti_random.tex <==

\multirow{3}{*}{Random} & CSPN   & ? & ? & ? & ? \\
 & NLSPN   & ? & ? & ? & ? \\
 & Ours & ? & ? & ? & ? \\\hline


==> tables/kitti_whole_table/kitti_whole_table.tex <==
\begin{table}
\centering
\resizebox{83.5mm}{18mm}{
\begin{tabular}{c|c|cccc}
\hline
Sample Method  & Method  & RMSE & IRMSE & MAE & IMAE 
\\ \hline
\input{tables/kitti_whole_table/kitti_lidar}
\input{tables/kitti_whole_table/kitti_keypoint}
\input{tables/kitti_whole_table/kitti_random}
\end{tabular}

}
\caption{\textbf{Results on KITTI}. Numbers in \textbf{bold} are the best results.}   

\label{kitti_whole_table}
\end{table}

==> tables/nyu_eth.tex <==
\begin{table}
\centering
\resizebox{70mm}{!}{
\begin{tabular}{p{2cm}<{\centering} |p{2.5cm}<{\centering} p{2.5cm}<{\centering}}
\hline
Method & Keypoint & Random \\ \hline

NLSPN ~\cite{nlspn} & 0.158 / 43.3 & 0.229 / 38.8 \\ \hline
CSPN ~\cite{cspn}   & 0.158 / 43.3 & 0.229 / 38.8 \\ \hline
Ours                & 0.130 / 47.5 & 0.207 / 39.6 \\ \hline

\end{tabular}

}
\caption{\textbf{Comparison of different sampling methods on ETH3D.}
Evaluation results are $rel / \delta_{1.02}$. 
Networks are trained on NYUv2~\cite{nyuv2} with 800 keypoint or random sampled points.
Networks trained on Keypoint sampling have obvious improvement.}   
\label{tab:nyuv2_eth_table}
\end{table}


==> tables/nyuv2_key_800.tex <==
\begin{table}
\centering
\resizebox{83.5mm}{8mm}{
\begin{tabular}{c|cc|cccc}
\hline
Method  & RMSE & REL & $\delta_{1.02}$ & $\delta_{1.05}$ & $\delta_{1.10}$ & $\delta_{1.25}$ 
\\ \hline
CSPN ~\cite{cspn}  & 0.220	& 0.0432 & 55.3 &	78.34 &	88.94 & 96.11\\ \hline
NLSPN ~\cite{nlspn}  & ? & ? & ? &	? &	? & ?\\ \hline
Ours & \textbf{0.159} & \textbf{0.0306} & \textbf{64.8} & \textbf{84.38} & \textbf{92.92} & \textbf{98.1}\\ \hline

\end{tabular}

}
\caption{\textbf{Results on NYUv2 with 800 keypoints input}.  Our method get much better performance on all the metrics than CSPN\cite{cspn}.}   

\label{tab:nyuv2_key_800_table}
\end{table}

==> tables/nyuv2_whole_table/nyuv2_different_sample.tex <==

\multirow{2}{*}{K} 
& \multirow{2}{*}{R} 
& CSPN & 0.131	& 0.020 & 71.1 & 92.3 &	97.1  \\ 
& & Ours & 0.103	& 0.013 & 87.1 & 95.0 &	97.7  \\ \midrule
\multirow{2}{*}{R}
& \multirow{2}{*}{K}
& CSPN & 1.176	& 0.286 & 46.7 & 62.5 &	71.6 \\ 
& & Ours & 0.380 & 0.084 & 50.6 & 68.8 & 79.5 \\


==> tables/nyuv2_whole_table/nyuv2_keypoint.tex <==
\multirow{3}{*}{K} &
\multirow{3}{*}{K} & 
   CSPN     & 0.220 & 0.043 & 55.3 & 78.3 &	88.9 \\
&& NLSPN    & 0.179 & 0.036 & 60.3 & 80.8 & 90.9 \\
&& Ours     & \textbf{0.163} & \textbf{0.031} & \textbf{64.9} & \textbf{84.1} & \textbf{92.6} \\ \midrule


==> tables/nyuv2_whole_table/nyuv2_lidar.tex <==
\multirow{3}{*}{Lidar} & 
\multirow{3}{*}{Lidar} & 
     CSPN   & ? & ? & ? & ? & ? & ? \\
&  & NLSPN  & ? & ? & ? & ? & ? & ? \\
&  & Ours   & ? & ? & ? & ? & ? & ? \\ \midrule

==> tables/nyuv2_whole_table/nyuv2_random.tex <==

\multirow{3}{*}{R} & \multirow{3}{*}{R} & CSPN  & 0.105	& 0.014 & 86.3 & 95.0 &	97.8  \\
&  & NLSPN  & \textbf{0.098} & \textbf{0.012} & \textbf{88.6} & \textbf{95.6} & \textbf{98.0} \\
&  & Ours & 0.102  & 0.013  & 86.4 & 94.6 &	97.6  \\ \hline


==> tex/experiments_backup.tex <==
\section{Experiments}
In this section, we evaluate robustness of networks trained on keypoint, random sampling, and compare our SSPN with other spatial propagation networks given keypoint sampled depth and sparse points from SfM (Sec. ~\ref{sec:depth_completion_keypoints}).
Then we conduct ablation studies to verify the effectiveness of each proposed component and compare performance of networks trained with different sampling methods when given sparse point clouds. (Sec.~\ref{sec:ablation_studies_experiments}).
Finally, we compare our method to other depth completion pipelines given uniform depth input (Sec.~\ref{sec:Previous_evaluation_experiment}). 

% In experiments, we show that keypoint sampling is a superior sampling method than random sampling, and our SSPN outperforms other spatial propagation methods given keypoint sampled depth or sparse points from SfM (Sec. ~\ref{sec:depth_completion_keypoints}).
% Two ablation studies show the effectiveness of each proposed component and improvement of keypoint sampling compared to random sampling given sparse point clouds (Sec.~\ref{sec:ablation_studies_experiments}).
% Also, we show that our method still have ... performance given uniform depth input compared to previous depth completion pipelines (Sec.~\ref{sec:Previous_evaluation_experiment}). 
\input{figures/eth3d_depth}
\noindent
\textbf{Evaluation Metrics}
For depth completion, we follows metrics of ~\cite{sparse_to_dense}, but select more strict inlier threshold 1.02, 1.05, 1.10, and 1.25 to have a better accuracy comparison;
For Lidar depth completion, we choose the official metrics of KITTI ~\cite{kitti};
For point clouds evaluation, we use the standard metrics following ETH3D~\cite{eth3d}. 

\subsection{Depth Completion from Sparse Keypoints}
\label{sec:depth_completion_keypoints}
% We compare our method with CSPN~\cite{cspn} and NLSPN~\cite{nlspn} given 800 input points sampled from random and keypoint strategies.
We evaluate our SSPN, CSPN~\cite{cspn}, NLSPN~\cite{nlspn} on NYUv2~\cite{nyuv2} with 800 input points using keypoint and random sampling.
We then compare performance of these three pipelines on ETH3D~\cite{eth3d} given sparse points generated by COLMAP~\cite{colmap}.
With the depth prediction on ETH3D, we fuse point clouds for each propagation method, and compare them with outdated existing MVS approaches, e.g. Gipuma ~\cite{Red_black_scheme}. 
% Also, we show that 
\newline

\noindent
\textbf{NYU V2 completion from sparse ground truth depth}
\label{sec:4.1.1}

\noindent
\textit{NYU Depth V2}~\cite{nyuv2} consists of paired RGB images and dense depth maps collected from 464 different indoor scenes with a Microsoft Kinect. 
Following~\cite{sparse_to_dense}, the training sets are generated by sampling evenly from raw video sequences on training splits, and official test split of 654 densely labeled images are used for evaluation.
All ground truth depth are obtained by filling missing values using original acquired raw depth.
To exclude depth artifact on borders, we center crop the original frames to get frames with a resolution of 448 x 608. 

% \Derek{1. Training on keypoint samples is essential for inference on keypoint samples and is also effective for inference on random samples.
% 2. Our method completes depth from keypoint samples much better than CSPN and NLSPN.}
Table~\ref{tab:nyuv2_whole_table} provides the results under different sampling methods.
We show that training on keypoint samples is essential for inference on keypoint samples and is also effective for inference on random samples, while the other way doesn't have reliable prediction.
Also, our method significantly outperforms when depth is available only on keypoint locations, which requires more effective long-range propagation.
% Given random sampled points, NLSPN performs best, while CSPN and our method also have similar performance.
% Meanwhile, our method significantly outperforms when depth is available only on keypoint locations, which requires more effective long-range propagation.
Fig.~\ref{fig:nyuv2_qualitative_figure} shows that our method predicts reliable depth on textureless areas given keypoints input.
% Also, training on keypoint and testing on uniform works much better than the other way.  
% This is an example of where training in the hard case is better.
\newline
\input{tables/eth3d_depth}
\input{tables/eth3d_pc}
\input{figures/eth3d_pc}

\noindent
\textbf{ETH3D completion from sparse SfM points}

% We first conduct a depth evaluation given sparse point from SFM for our pipeline, CSPN~\cite{cspn} and NLSPN~\cite{nlspn}.
% Then we compare the fused point clouds from each depth completion algorithm with a conventional MVS pipeline Gipuma~\cite{Red_black_scheme}.

% We show that our network trained using keypoint sampling could predict reliable depth on ETH3D\cite{eth3d}. 
% Our method could reconstruct point clouds that are comparable to conventional MVS algorithms in a loose threshold with a shorter running time.

\noindent
\textit{ETH3D}\cite{eth3d} is a challenging MVS dataset that provides stereo images,  sparse point clouds generated by COLMAP SFM\cite{colmap}, and  ground truth point clouds captured by laser scanners.
To have a reasonable evaluation time, we resize the high resolution images to 960 x 640.

Due to the highly overlapped images within each scene, ETH3D is not suitable for training of single view depth completion algorithms. 
Therefore, we directly compare networks that trained on NYUv2 with keypoint sampling in Table \ref{tab:eth3d_depth_table}. 
Our method shows better results on all metrics except for RMSE compared to CSPN and NLSPN. 
% SSPN achieves great improvement on all metrics except for RMSE. 
In Fig \ref{fig:eth3d_depth_figure}, we present some qualitative examples. 
ETH3D completion is challenging because the input depth are sparse, and contain incorrect values, so CSPN has blocky artifact, and NLSPN is wrongly guided by the input. 
However, even under such challenges, SSPN still has decent prediction.

\noindent
\textbf{ETH3D point cloud evaluation}

We fuse the point clouds using depth prediction from each method by checking the absolute depth distance between each reference image with the source views following the fusion strategy of ~\cite{Red_black_scheme, Schnberger2016PixelwiseVS}.
We set a absolute depth threshold as 0.1 meter and consistency view as 2.
These point clouds are compared to a traditional MVS algorithm Gipuma\cite{Red_black_scheme} in Table \ref{tab:eth3d_pc_table} under MVS standard.
From the table, Gipuma gains high accuracy with a low completeness trade-off, so under 5 cm, our method and NLSPN get higher F1 scores.
Although we accomplish depth prediction more accurate than NLSPN's, during the point cloud fusion stage, which removes much noisy depth, our advantages on depth maps doesn't transit to the equivalent improvement on point clouds.
We show several comparison of point clouds from our method and a state-of-the-art method ACMM~\cite{ACMM} in Fig \ref{fig:eth3d_pc}. 
From the results, our fused point clouds are not as accurate as ACMM, but it manages to recover textureless areas where ACMM fails. 
% Note that we are trained on NYUv2, so this is a cross-dataset performance. 
CSPN~\cite{cspn}, NLSPN~\cite{nlspn}, and our SSPN achieves 4.8, 7.3, 4.6 FPS, with a peak memory usage of 2443MB, 6985MB, 6983MB separately when testing on Quadro RTX 6000 under a resolution of 960 x 640.

\subsection{Ablation Studies}
\label{sec:ablation_studies_experiments}
% we conduct experiments to show each our component's contribution towards the improvement over CSPN~\cite{cspn}.
Table~\ref{tab:ablation_study_table} evaluates the contribution of each component of our network and Table~\ref{tab:nyuv2_eth_table} evaluates the improvement of keypoint sampling over random sampling.
\input{tables/ablation_study}

\noindent
\textbf{Importance of Dilation Kernel}
As shown on Fig.~\ref{fig:receptive_field_figure}, the use of dilation kernel would significantly improve the receptive field with exactly same resources. 
By comparing "w/ ctf" and "w/ dilation \& ctf" in Table \ref{tab:ablation_study_table}, the use of dilation kernel gains 13\% on $\delta_{1.02}$.

\noindent
\textbf{Importance of Coarse-to-fine Network}
Coarse-to-fine network further expands the receptive fields. 
By comparing "w/ dilation" and "w/ dilation \& ctf" in Table~\ref{tab:ablation_study_table},  the use of coarse-to-fine network boost a 17.6\% improvement on $\delta_{1.02}$.

\input{tables/nyu_eth}
\noindent
\textbf{Importance of Keypoint Sampling}
To compare the effect of keypoint sampling, we evaluate our and NLSPN ~\cite{nlspn} performance on ETH3D when trained with two sampling methods on NYUv2 in Table~\ref{tab:nyuv2_eth_table}. 
Keypoint sampling training achieves a 35\% improvement on REL and 15\% improvement on $\delta_{1.02}$ compared to random sampling.

\subsection{Comparison with uniform depth input}
\label{sec:Previous_evaluation_experiment}
We compare our method to other depth completion pipelines ~\cite{deep_lidar, depth_normal, cspn, cspn++, nlspn} on KITTI depth completion task and resized NYUv2 with 500 random sampled input.

\input{tables/kitti_test}
\input{tables/nyuv2_uniform_500}

\noindent
\textit{KITTI} \cite{kitti} contains over 93k RGB images and Lidar depth input, and ground truth depth pairs. 
Following ~\cite{nlspn}, we only use the bottom crop (1216 x 240) of the pairs for training.

Table ~\ref{tab:kitti_test} presents the testing performance acquired from the official website.
Although our methods are focused on the sparse point inputs, we still achieve on-par MAE and IMAE results with state of the art.

\noindent
\textbf{Resized NYUv2}
% To have a comparison to all previous depth completion methods, we first use a resolution of 304 x 228 with 500 random sampling points following \cite{sparse_to_dense}. 
% The results are shown at Table \ref{nyuv2_uniform_500}
Table ~\ref{tab:nyuv2_uniform_500} presents the comparison under a resolution of 304 x 228 with 500 random sampling points following ~\cite{sparse_to_dense}. 
Given uniformly sampled points, NLSPN is the best, while our method is a close second. 


==> tex/limitation.tex <==
\section{Limitation}

==> tex/results.tex <==
\section{Results}
We evaluate our 

\subsection{Key Point Datasets Results}

\noindent
\textbf{NYUv2}

\noindent
\textbf{ETH3D}

\subsection{Lidar Depth Datasets Results}

\noindent
\textbf{KITTI}

\noindent
\textbf{NYUv2}


\subsection{Ablation Studies}

\noindent
\textbf{Importance of Diffusion Kernel}

\noindent
\textbf{Importance of Coarse-to-fine Network}

% \noindent
% \textbf{Influence of Number of Key Points}

==> tex/save.tex <==
\Replace{
    Existing literature~\cite{deep_depth_completion,deep_lidar,cspn,nlspn,cspn++}  mainly focuses on LiDAR completion, which assumes that the captured sparse depths follow rough uniform sampling over the image. 
    In training time, these methods simulate LiDAR by uniformly sampling fixed number of keypoints with known values, and have been evolved to interpolate values between the semi-dense known depth input. 
    Because small local neighborhoods are mostly guaranteed to contain sparse depth point, existing works have evolved to use encoder-decoder architecture that squeezes semi-dense depth map into smaller spatial domain with deep contexts, and unsqueezes them into a complete dense depth map. }
    
    \Replace{
    On the other hand, not much attention has given on the sparse map inputs, which typically has clustered distribution of sparse points near the feature detection points, such as SIFT~\cite{SIFT} or FAST~\cite{FAST}. 
    Unlike the semi-dense LiDAR depth input, clustered distribution contains larger regions without known depth values, which makes the encoder-decoder like architectures fail to effectively interpolate nearby depth values due to the limited reachability. }
    \input{figures/cspn_failure}
    
    
    \Replace{    
    In this paper, we present a way to learn to perform depth completion on both LiDAR based depth as well as sparse maps. 
    Our method adopts the Convolutional Sparse Propagation Network (CSPN) which learns to propagate near by depth values based on affinity matrix. 
    We focus on increasing the reachability of the spatial propagation by using the insights from the diffusion based kernels~\cite{Red_black_scheme} which is known to have faster propagation given same number of propagation iterations, and by using coarse-to-fine architecture that lets propagation to initially run on smaller spatial domain for even larger propagation coverage.  Moreover, we propose a way to simulate sparse map input by sampling depth points using SIFT keypoint detector. Instead of using uniform sampling from the known depth values, we perform SIFT keypoint detector to extract feature point locations in the image, and extracts the corresponding depth values in the detected feature point location.}
    
    \Replace{
    We validate our work using experiments. We first extensively show our method's performance compared to the baseline methods in the existing datasets, such as NYUv2~\cite{nyuv2} and KITTI~\cite{kitti} benchmarks to show how our method performs in the LiDAR completion. 
    Next, we show that our model trained on keypoint based sampling outperforms existing spatial propagation network models~\cite{cspn,nlspn} by a huge margin, and on-par when trained with uniform sampling or simulated LiDAR sampling. 
    Finally, we validate our model trained with keypoint based sampling strategy, by comparing it to the challenging multi-view stereo dataset, ETH3D High-res benchmark.  }
    
    \input{figures/network}
    % \input{figures/eth3d_pc}
    \Replace{
    In summary, our main \textbf{contributions} of the paper are:
    \begin{itemize}
        \vspace{-0.5em}
        \item  \textbf{Proposing Diffusion based SPN kernel} that covers larger propagation area at the same algorithmic complexity. 
        \vspace{-0.5em}
        \item \textbf{Coarse to Fine architecture} which further extends affinity propagation reachability. 
        \vspace{-0.5em}
        \item \textbf{Key Point based sampling} that trains the model suitable for the depth completion for the sparse map inputs. 
        \vspace{-1.0em}
    \end{itemize}}
